Characterising resource management performance in Kubernetes

A key challenge for supporting elastic behaviour in cloud systems is to achieve a good performance in automated (de-)provisioning and scheduling of computing resources. One of the key aspects that can be significant is the overheads associated with deploying, terminating and maintaining resources. Therefore, due to their lower start up and termination overhead, containers are rapidly replacing Virtual Machines (VMs) in many cloud deployments, as the computation instance of choice. In this paper, we analyse the performance of Kubernetes achieved through a Petri net-based performance model. Kubernetes is a container management system for a distributed cluster environment. Our model can be characterised using data from a Kubernetes deployment, and can be exploited for supporting capacity planning and designing Kubernetes-based elastic applications.

==> figures/TreeV3.tex <==
<?xml version="1.0" encoding="UTF-8"?>
<dia:diagram xmlns:dia="http://www.lysator.liu.se/~alla/dia/">
  <dia:diagramdata>
    <dia:attribute name="background">
      <dia:color val="#ffffff"/>
    </dia:attribute>
    <dia:attribute name="pagebreak">
      <dia:color val="#000099"/>
    </dia:attribute>
    <dia:attribute name="paper">
      <dia:composite type="paper">
        <dia:attribute name="name">
          <dia:string>#A4#</dia:string>
        </dia:attribute>
        <dia:attribute name="tmargin">
          <dia:real val="2.8222000598907471"/>
        </dia:attribute>
        <dia:attribute name="bmargin">
          <dia:real val="2.8222000598907471"/>
        </dia:attribute>
        <dia:attribute name="lmargin">
          <dia:real val="2.8222000598907471"/>
        </dia:attribute>
        <dia:attribute name="rmargin">
          <dia:real val="2.8222000598907471"/>
        </dia:attribute>
        <dia:attribute name="is_portrait">
          <dia:boolean val="true"/>
        </dia:attribute>
        <dia:attribute name="scaling">
          <dia:real val="1"/>
        </dia:attribute>
        <dia:attribute name="fitto">
          <dia:boolean val="false"/>
        </dia:attribute>
      </dia:composite>
    </dia:attribute>
    <dia:attribute name="grid">
      <dia:composite type="grid">
        <dia:attribute name="width_x">
          <dia:real val="1"/>
        </dia:attribute>
        <dia:attribute name="width_y">
          <dia:real val="1"/>
        </dia:attribute>
        <dia:attribute name="visible_x">
          <dia:int val="1"/>
        </dia:attribute>
        <dia:attribute name="visible_y">
          <dia:int val="1"/>
        </dia:attribute>
        <dia:composite type="color"/>
      </dia:composite>
    </dia:attribute>
    <dia:attribute name="color">
      <dia:color val="#d8e5e5"/>
    </dia:attribute>
    <dia:attribute name="guides">
      <dia:composite type="guides">
        <dia:attribute name="hguides"/>
        <dia:attribute name="vguides"/>
      </dia:composite>
    </dia:attribute>
  </dia:diagramdata>
  <dia:layer name="Fondo" visible="true" active="true">
    <dia:object type="Standard - Ellipse" version="0" id="O0">
      <dia:attribute name="obj_pos">
        <dia:point val="35.2902,8.42337"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="35.2402,8.37337;41.8785,11.4234"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="35.2902,8.42337"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="6.5383412568924086"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="2.9499999999999957"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#90ee90"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Ellipse" version="0" id="O1">
      <dia:attribute name="obj_pos">
        <dia:point val="19.3014,8.52746"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="19.2514,8.47746;25.8897,11.5275"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="19.3014,8.52746"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="6.5383412568924086"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="2.9499999999999957"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#90ee90"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Flowchart - Box" version="0" id="O2">
      <dia:attribute name="obj_pos">
        <dia:point val="23.3257,-8.01388"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="23.2757,-8.06388;28.0532,-6.06388"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="23.3257,-8.01388"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="4.6775000014901158"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="1.9000000014901162"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#add8e6"/>
      </dia:attribute>
      <dia:attribute name="show_background">
        <dia:boolean val="true"/>
      </dia:attribute>
      <dia:attribute name="padding">
        <dia:real val="0.5"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Application#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="25.6645,-6.86888"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="1"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
    </dia:object>
    <dia:object type="Flowchart - Box" version="0" id="O3">
      <dia:attribute name="obj_pos">
        <dia:point val="13.755,-3.37125"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="13.705,-3.42125;21.295,-1.42125"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="13.755,-3.37125"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="7.4900000014901158"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="1.9000000014901162"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#add8e6"/>
      </dia:attribute>
      <dia:attribute name="show_background">
        <dia:boolean val="true"/>
      </dia:attribute>
      <dia:attribute name="padding">
        <dia:real val="0.5"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#CPU or I/O intensive#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="17.5,-2.22625"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="1"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
    </dia:object>
    <dia:object type="Flowchart - Box" version="0" id="O4">
      <dia:attribute name="obj_pos">
        <dia:point val="12.326,4.68688"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="12.276,4.63688;15.891,6.63688"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="12.326,4.68688"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="3.5150000000000001"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="1.9000000014901162"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#add8e6"/>
      </dia:attribute>
      <dia:attribute name="show_background">
        <dia:boolean val="true"/>
      </dia:attribute>
      <dia:attribute name="padding">
        <dia:real val="0.5"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#C&gt;= n#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="14.0835,5.83188"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="1"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
    </dia:object>
    <dia:object type="Flowchart - Box" version="0" id="O5">
      <dia:attribute name="obj_pos">
        <dia:point val="20.916,4.68688"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="20.866,4.63688;24.481,6.63688"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="20.916,4.68688"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="3.5150000000000001"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="1.9000000014901162"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#add8e6"/>
      </dia:attribute>
      <dia:attribute name="show_background">
        <dia:boolean val="true"/>
      </dia:attribute>
      <dia:attribute name="padding">
        <dia:real val="0.5"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#C &lt; n#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="22.6735,5.83188"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="1"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
    </dia:object>
    <dia:object type="Flowchart - Box" version="0" id="O6">
      <dia:attribute name="obj_pos">
        <dia:point val="30.7663,0.5075"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="30.7163,0.4575;46.5888,4.0575"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="30.7663,0.5075"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="15.772500001490116"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="3.5000000014901165"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#add8e6"/>
      </dia:attribute>
      <dia:attribute name="show_background">
        <dia:boolean val="true"/>
      </dia:attribute>
      <dia:attribute name="padding">
        <dia:real val="0.5"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Job &amp;
Deployment Overhead &lt; Execution Overhead
(Eq. 1)#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="38.6526,1.6525"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="1"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
    </dia:object>
    <dia:object type="Flowchart - Box" version="0" id="O7">
      <dia:attribute name="obj_pos">
        <dia:point val="25.335,0.9575"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="25.285,0.9075;28.855,2.9075"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="25.335,0.9575"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="3.4700000014901162"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="1.9000000014901162"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#add8e6"/>
      </dia:attribute>
      <dia:attribute name="show_background">
        <dia:boolean val="true"/>
      </dia:attribute>
      <dia:attribute name="padding">
        <dia:real val="0.5"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Service#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="27.07,2.1025"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="1"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
    </dia:object>
    <dia:object type="Flowchart - Box" version="0" id="O8">
      <dia:attribute name="obj_pos">
        <dia:point val="27.775,-3.32125"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="27.725,-3.37125;35.275,-1.37125"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="27.775,-3.32125"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="7.4499999999999993"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="1.9000000014901162"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#add8e6"/>
      </dia:attribute>
      <dia:attribute name="show_background">
        <dia:boolean val="true"/>
      </dia:attribute>
      <dia:attribute name="padding">
        <dia:real val="0.5"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Network Intensive#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="31.5,-2.17625"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="1"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O9">
      <dia:attribute name="obj_pos">
        <dia:point val="38.6526,2.2575"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="38.6526,1.6625;38.6526,2.4075"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>##</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="38.6526,2.2575"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O6" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O10">
      <dia:attribute name="obj_pos">
        <dia:point val="23.9054,-6.06361"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="19.1909,-6.13179;23.9736,-3.35334"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="23.9054,-6.06361"/>
        <dia:point val="19.2591,-3.42152"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O2" connection="16"/>
        <dia:connection handle="1" to="O3" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O11">
      <dia:attribute name="obj_pos">
        <dia:point val="26.9075,-6.06429"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="26.8372,-6.13459;30.3273,-3.30054"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="26.9075,-6.06429"/>
        <dia:point val="30.257,-3.37084"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O2" connection="16"/>
        <dia:connection handle="1" to="O8" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O12">
      <dia:attribute name="obj_pos">
        <dia:point val="30.465,-1.37155"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="28.0343,-1.44225;30.5357,0.978502"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="30.465,-1.37155"/>
        <dia:point val="28.105,0.907802"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O8" connection="16"/>
        <dia:connection handle="1" to="O7" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O13">
      <dia:attribute name="obj_pos">
        <dia:point val="33.0445,-1.37171"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="32.9754,-1.44085;35.9408,0.527012"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="33.0445,-1.37171"/>
        <dia:point val="35.8717,0.45787"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O8" connection="16"/>
        <dia:connection handle="1" to="O6" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O14">
      <dia:attribute name="obj_pos">
        <dia:point val="17.0761,-1.42136"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="14.4419,-1.48691;17.1416,4.70254"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="17.0761,-1.42136"/>
        <dia:point val="14.5074,4.63699"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O3" connection="16"/>
        <dia:connection handle="1" to="O4" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O15">
      <dia:attribute name="obj_pos">
        <dia:point val="18.1419,-1.42136"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="18.0729,-1.49045;22.1006,4.70608"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="18.1419,-1.42136"/>
        <dia:point val="22.0315,4.63699"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O3" connection="16"/>
        <dia:connection handle="1" to="O5" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O16">
      <dia:attribute name="obj_pos">
        <dia:point val="25.2866,2.41965"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="15.8292,2.35779;25.3484,5.17965"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="25.2866,2.41965"/>
        <dia:point val="15.8911,5.11779"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O7" connection="16"/>
        <dia:connection handle="1" to="O4" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O17">
      <dia:attribute name="obj_pos">
        <dia:point val="38.6306,4.05672"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="38.5274,4.00612;38.6812,8.4249"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="38.6306,4.05672"/>
        <dia:point val="38.578,8.3743"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O6" connection="16"/>
        <dia:connection handle="1" to="O0" connection="8"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O18">
      <dia:attribute name="obj_pos">
        <dia:point val="25.8909,2.90768"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="23.7821,2.8372;25.9614,4.70718"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="25.8909,2.90768"/>
        <dia:point val="23.8526,4.63671"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O7" connection="16"/>
        <dia:connection handle="1" to="O5" connection="16"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O19">
      <dia:attribute name="obj_pos">
        <dia:point val="14.0795,6.63646"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="14.0219,6.58626;14.1297,8.56388"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="14.0795,6.63646"/>
        <dia:point val="14.072,8.51368"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O4" connection="16"/>
        <dia:connection handle="1" to="O21" connection="8"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Line" version="0" id="O20">
      <dia:attribute name="obj_pos">
        <dia:point val="22.6499,6.63715"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="22.5553,6.58599;22.7011,8.52898"/>
      </dia:attribute>
      <dia:attribute name="conn_endpoints">
        <dia:point val="22.6499,6.63715"/>
        <dia:point val="22.6065,8.47782"/>
      </dia:attribute>
      <dia:attribute name="numcp">
        <dia:int val="1"/>
      </dia:attribute>
      <dia:connections>
        <dia:connection handle="0" to="O5" connection="16"/>
        <dia:connection handle="1" to="O1" connection="8"/>
      </dia:connections>
    </dia:object>
    <dia:object type="Standard - Ellipse" version="0" id="O21">
      <dia:attribute name="obj_pos">
        <dia:point val="10.7968,8.56194"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="10.7468,8.51194;17.3852,11.5619"/>
      </dia:attribute>
      <dia:attribute name="elem_corner">
        <dia:point val="10.7968,8.56194"/>
      </dia:attribute>
      <dia:attribute name="elem_width">
        <dia:real val="6.5383412568924086"/>
      </dia:attribute>
      <dia:attribute name="elem_height">
        <dia:real val="2.9499999999999957"/>
      </dia:attribute>
      <dia:attribute name="border_width">
        <dia:real val="0.10000000149011612"/>
      </dia:attribute>
      <dia:attribute name="inner_color">
        <dia:color val="#90ee90"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O22">
      <dia:attribute name="obj_pos">
        <dia:point val="11.261,9.82872"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="11.261,9.23372;16.871,9.97872"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Group Containers#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="11.261,9.82872"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O23">
      <dia:attribute name="obj_pos">
        <dia:point val="12.7385,10.7269"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="12.7385,10.1319;15.3935,10.8769"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#rho=n/C#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="12.7385,10.7269"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O24">
      <dia:attribute name="obj_pos">
        <dia:point val="20.1696,9.82872"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="20.1696,9.23372;25.2521,9.97872"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Split Containers#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="20.1696,9.82872"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O25">
      <dia:attribute name="obj_pos">
        <dia:point val="21.7134,10.7269"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="21.7134,10.1319;23.7084,10.8769"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#rho=1#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="21.7134,10.7269"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O26">
      <dia:attribute name="obj_pos">
        <dia:point val="35.9151,9.82872"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="35.9151,9.23372;40.9976,9.97872"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Split Containers#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="35.9151,9.82872"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O27">
      <dia:attribute name="obj_pos">
        <dia:point val="37.4588,10.7269"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="37.4588,10.1319;39.4538,10.8769"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#rho=1#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="37.4588,10.7269"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O28">
      <dia:attribute name="obj_pos">
        <dia:point val="12.4672,12.3168"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="12.4672,11.7218;15.6647,12.4668"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Rule no. 1#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="12.4672,12.3168"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O29">
      <dia:attribute name="obj_pos">
        <dia:point val="21.1121,12.3168"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="21.1121,11.7218;24.3096,12.4668"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Rule no. 2#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="21.1121,12.3168"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
    <dia:object type="Standard - Text" version="1" id="O30">
      <dia:attribute name="obj_pos">
        <dia:point val="36.8576,12.3168"/>
      </dia:attribute>
      <dia:attribute name="obj_bb">
        <dia:rectangle val="36.8576,11.7218;40.0551,12.4668"/>
      </dia:attribute>
      <dia:attribute name="text">
        <dia:composite type="text">
          <dia:attribute name="string">
            <dia:string>#Rule no. 2#</dia:string>
          </dia:attribute>
          <dia:attribute name="font">
            <dia:font family="sans" style="0" name="Helvetica"/>
          </dia:attribute>
          <dia:attribute name="height">
            <dia:real val="0.80000000000000004"/>
          </dia:attribute>
          <dia:attribute name="pos">
            <dia:point val="36.8576,12.3168"/>
          </dia:attribute>
          <dia:attribute name="color">
            <dia:color val="#000000"/>
          </dia:attribute>
          <dia:attribute name="alignment">
            <dia:enum val="0"/>
          </dia:attribute>
        </dia:composite>
      </dia:attribute>
      <dia:attribute name="valign">
        <dia:enum val="3"/>
      </dia:attribute>
    </dia:object>
  </dia:layer>
</dia:diagram>


==> files/Background.tex <==
%\subsection{Petri nets}
%\label{sec:background}
A Petri Net~\cite{murata1989petri} is one of several formal models for the description and the analysis of distributed, parallel or concurrent computing systems. It can be seen as a bipartite graph, where nodes
can be of two types, either places or transitions; and arcs connect a transition with a place or viceversa.
A place is often represented by a circle, whereas a transition by a rectangle.
Besides, places can contain a (discrete) number of tokens (a token is typically represented as \emph{[]}).
In order to model a system, all these constituents can represent the dynamics of a system in a number of different ways.
For instance, a transition can model a system action, and a place can represent a state, arcs can represent that each transition
has a certain number of input and output places, 
modelling pre-conditions and postconditions of the system action. 
Tokens move from one pre-condition state to a post-condition state, when the involved transition is fired. In this way, it can be used
to capture the evolution of system semantics.
In this paper, we are making use of a particular type of Petri nets called Reference Nets.
Reference Nets belong to the class of High-Level Petri nets (HLPN)~\cite{kummer2004extensible}.
An HLPN is a Petri net whose tokens are represented by data structures or even objects. The pre-conditions 
of an HLPN can be labeled by expressions that identify states defined by the value of tokens. Besides, post-conditions can be labeled by expressions that define state changes by the modification of token values.
In this way, HLPNs provide a more concise representation than ordinary Petri nets.
In essence, Reference nets extend High-Level Petri nets  with some characteristics that support the construction of hierarchical models, by allowing a token to be a net itself, creating hierarchies of nets. The nets forming part of such hierarchies can communicate by means of synchronous channels.  
Synchronous channels can be seen as a sophisticated way of message passing communication, but with a richer semantics based  in the unification mechanism.
A synchronous channel engages two transitions (typically from different nets) that, by means of the channel, fire
(synchronize) simultaneously. The channel can also accommodate variables and it has two main roles:
The \emph{uplink} or callee role, at the subordinated instance net, which servers requests.
The \emph{downlink} or caller role, at the parent net, which makes use of the channel to both synchronize and
call the subordinate instance. 

Channel communication and hierarchies provide the way to describe finely grained complex behaviors in the form of nested Petri nets. 
The usefulness of net instances lies in the fact that they can represent behaviors that can be moved to different execution environments. 
The inscription language of Reference nets have also been extended to include
tuples, which can be used for representing a group of related values or variables in a single token. 
A net instance can be influenced by the net that holds it, called System net, and such influence is accomplished by means of the synchronous channels mechanism.


The execution of a HLPN specification requires to find bindings, i.e. mapping of variables used in
are expressions to specific values. 

Reference Nets can be interpreted by Renew~\footnote{{\tt http://www.renew.de}}~\cite{kummer2004extensible}, a Java-based Reference net interpreter and graphical modeling tool. The way Renew binds variables  to values is by unification,  the same mechanism used by logic programming languages such as Prolog. In HLPNs, when a transition fires, then its expression is evaluated and tokens are moved according to the result. Furthermore, Reference Nets incorporate some characteristics from object-oriented languages: Reference Nets support the creation of net instances dynamically, and transitions also support the inclusion of inscriptions, including Java inscriptions. Therefore, Reference Nets also support the creation of Java objects, and Java method
invocations inside a net. 
They also incorporate the assignment operator  ``=", and it can be used to define (assign) the value of variables.


Reference Nets can hold two kinds of tokens: Valued tokens and tokens which correspond to a reference to a PN instance. By default, an arc will transport a black token, denoted by {\tt []}. In case an inscription is added to an arc, that inscription will be evaluated and the result will
determine which kind of token is moved.





\begin{figure}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \centering  
\includegraphics[width=1\columnwidth]{figures/consumerProviders.pdf}
\caption{A Reference net model that represents a {\tt Service Consumer} and a {\tt Resource Provider}. References to  {\tt Resources} net instances are managed by the consumer to provide data and collect results,  and providers to manage resources.}
\label{introRenew}
\end{figure}
  
 In order to illustrate the main concepts of Reference Nets,
Figure~\ref{introRenew} depicts a Reference net Nodel that
represents a {\tt Resource Consumer} and a {\tt Resource
Provider} with allocating capacity of two
resources. Services are required with a QoS and
data to be processed when {\tt Consumer} invokes the {\tt match}
channel. Communication happens when unification of variables is
possible. In the state represented in the figure, the transition
labelled with the downlink {\tt this:match(request, Qos, inputData)} channel in the {\tt Consumer}
can synchronise with transitions labelled with uplinks {\tt :match(service, QoS,Res)}  in the {\tt Resource Provider}. 
Figure~\ref{introRenew} shows one allocated resource providing service, and  one available resource. There are two possible bindings with {\tt data1} and {\tt data2}, but there is only one available resource, and therefore transitions with downlink and uplink will be synchronously fired with one of the two possible bindings.





==> files/Kubernetes.tex <==
Kubernetes \cite{Burns:2016} is an open source platform that abstracts and automates the deployment of applications across a number of distributed, computational resources. Kubernetes makes use of container technologies in order to manage and provide computational resources. In this section, we will briefly analyse container technologies and Kubernetes in particular.


\subsection{Container approach}
\label{sec:containerapproach}

VMs have been one of the first and most important cloud computational resources.  A VM is a piece of software that emulates a hardware computing system and typically multiple VMs share the same hardware to be executed. The emulation is accomplished by a hypervisor. Hypervisors are responsible for dividing the hardware of the host physical machine, so that it can be used by the OS inside each VM. Therefore, applications that run inside a VM can accomplish calls to their own OS inside the VM, and then their virtual kernel executes instructions on the physical CPU of the host machine by means of the hypervisor. 

One of the most important benefits of using VMs is the full isolation they achieve: VMs on the same host physical machine share the same hardware, but they are completely isolated. Nevertheless, VM utilization can sometimes be difficult to achieve, e.g.  when the applications to be run do not consume all the resources of a VM. Developers can therefore can try to map multiple applications onto the same VM. In this case, applications would not be isolated. \emph{Containers}, on the other hand, represent a way to solve that isolation problem by improving utilization. A container can be seen as a set of processes where an application is executed in isolation. Multiple containers typically coexist on the same host machine, and each container in it uses the resources that the application on it consumes. Nevertheless, the degree of isolation achieved by VMs is still higher than the one achieved by containers, but containers have much less overhead. The reason for it is that all containers deployed in the same host machine share the same OS kernel, and therefore virtualization is not required. Furthermore, while a VM needs to boot up first before an application can be executed on it, a container is a group of processes whose execution can be initiated almost immediately. The isolation of containers is obtained by two Linux mechanisms: Linux namespaces and Linux Control Groups, which isolate the view of the system and limit the amount of computational resources, respectively.

Although container technologies were developed many years ago, they became popular with the emergence of Docker.
Docker containers became popular due to the fact that (i) they also help deploy library dependencies with the application
and (ii) the high portability of containers on  different platforms. 
A Docker container is a Docker image in execution. A Docker image contains an application and all the libraries required for its execution. In turn, Docker images are stored at the Docker registry, which also facilitates the availability of such images.


\subsection{Kubernetes Architecture}
\label{sec:kubarch}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.90\linewidth]{figures/architecture1.eps}
	\caption{Kubernetes architecture.}
	\label{fig:architecture1}
\end{figure}

Kubernetes is a system that allows developers to deploy and manage containerized applications. 
It is based on a master-slave architecture, with a particular emphasis on supporting a cluster of machines
where containers are executed. Applications are submitted to the master and Kubernetes, in turn, deploys them automatically across the worker nodes in containers. 
The communication between Kubernetes master \& slave nodes is realised through the \textit{kubelet} service.  This service must be executed on each machine in the Kubernetes cluster.  The node which acts as master can also carry out the role of a slave during execution.  The basic component architecture of Kubernetes is shown in Figure~\ref{fig:architecture1}.
As Kubernetes often works with Docker containers, the \textit{docker daemon} should be running on every machine in the cluster.  In addition, Kubernetes makes use of the \textit{etcd} project to have a key-value distributed storage system, in order to coordinate resources and to share configuration data of the cluster. The master node runs also  an API server, implemented with a RESTful interface, which gives an entry point to the cluster.  The API service is used as a proxy to expose the services which are executed inside the cluster to external applications/ users.

%%
In order to run an application, it has to be wrapped on one or more container images, then push (submit) these images to a container service registry, and then post a description of the application in the form of an application descriptor to the API server.
Then, Kubernetes will automatically retrieve the container images when the application is launched.
Instead of deploying containers individually, Kubernetes deploys \textit{pods}. A pod is an abstraction of a set of containers tightly coupled with some shared resources (the network interface and the storage system). Any OCI compliant container runtime engine could be used to execute containers in pods. With this abstraction, Kubernetes adds persistence to the deployment of single containers.  It is important to note two aspects of a pod: (i) a pod is scheduled to execute on one machine, with all containers inside the pod being deployed on the same machine; (ii)  a pod has a local IP address inside the cluster network, and all containers inside the pod share the same port space.  Therefore, each pod has a unique IP address in a flat shared networking space that allows bidirectional IP communications with all other pods and physical computers in the cluster.  The main implication of this is that two services which listen on the same port by default cannot be deployed inside a pod. 

 A pod can be replicated along several machines for scalability and fault tolerance purposes. When a service or a set of services are deployed over several machines, we can consider: (1) the  \textit{functional level} or application level involves exposing dependencies between the deployed services.  Different services need to be coordinated in order to provide a high level functionality.  An example of this kind of relationship is the deployment of a stream processing infrastructure (e.g. Apache Kafka, Storm, Zookeeper and HDFS for persistence) or the GuestBook example provided by Kubernetes, composed of a PHP frontend and a Redis master-slave system. (2) the \textit{operational level} or deployment level involves mapping services to physical machines, VMs, pods or containers.  It is platform dependant and must involve isolation between resources. Kubernetes primarily focuses on the operational/ deployment level.  A pod implements a service, and some coordination between different pods is achieved through the key-value distributed store provided by  {\em etcd}. Services running in others pods can be discovered through a DNS.  This approach imposes some restrictions to Kubernetes.  For instance, in the Guestbook example,  Kubernetes' scheduler cannot ensure that the three pods are deployed rightly, because Kubernetes does not manage the application level.

%There are some basic system services that can be deployed inside a Kubernetes cluster in order to provide high level functionalities.  They are deployed in an isolated namespace (kube-system).  In Figure~\ref{fig:architecture2}, we show the deployment of a Kubernetes cluster with logging and monitoring services.  With heapster service (provided by Kubernetes team), it is possible to monitorise the resource usage (RAM, CPU, Network and Filesystem).  We have included Prometheus to monitorise several response times and latencies in the cluster.  Both are connected to a Graphana dashboard.  The logging infrastructure consists on a fluentd service for collecting logs, a elastic search server and a Kibana dashboard.  The logs that fluentd collects are application logs.  In addition, Kubernetes has an specific DNS server that can be deployed as an addon inside a pod, an a web dashboard.
%
%
%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.80\linewidth]{figures/architecture2.eps}
%	\caption{Kubernetes deployment with several system services (DNS, monitorising and logging).}
%	\label{fig:architecture2}
%\end{figure}
%%Service + App pods -- relationship between these.






==> files/OldBackground.tex <==
\emph{Reference nets}~\cite{kummer02} are a special
class of high-level Petri nets (adhered to the
Nets-within-Nets~\cite{DBLP:conf/apn/Valk98} paradigm). 
A Petri net~\cite{murata89} can be seen as a bipartite graph, with a set of places,
a set of transitions, and arcs, where arcs connect a transition to a place or vice versa.
Places can contain a discrete number of marks, called \emph{tokens}, 
representing the dynamics of the petri net model.
In essence, Reference nets extend Petri nets by allowing a token to be a
net itself, creating hierarchies of nets. The nets forming part of such hierarchies
can communicate by means of synchronous channels. Furthermore, Reference nets
enable the creation of net instances dynamically, and they also support the inclusion of 
inscriptions, including Java inscriptions, in which the equality
operator ``=" can be used to influence the binding of variables.
The binding is similar to the way variables are used
in logic programming languages such as Prolog. 
Also, arcs can optionally have arc inscriptions, which are expressions:
if a transition fires, then its expression is evaluated and tokens are moved
according to the result. 

Besides, the
inscription language of Reference nets has also been designed to include
tuples. A tuple is a comma-separated list of both variables or expressions
that are enclosed in brackets. Tuples can be used for storing
a group of expressions or variable in a single token. 
Reference nets can hold two kinds of tokens: Valued tokens and tokens
which correspond to a reference. By default, an arc will transport a
black token, denoted by {\tt []}. In case an inscription is added to
an arc, that inscription will be evaluated and the result will
determine which kind of token is moved.

%Additionally, there are creation inscriptions that deal with the
%creation of net instances and synchronous channels. New net
%instances can be created by transitions that carry creation
%inscriptions, which consist of a variable name, a colon (:), the
%reserved word \emph{new} and the name of the net. Net instances can
%communicate with each other by means of synchronous channels. They
%synchronise two transitions which both fire atomically at the same
%time. Both transitions must agree on the name of the channel and on
%a set of parameters before they can synchronise. The initiating
%transition must have a special inscription -- called \emph{downlink}
%-- which makes a request to a designated subordinated net. A
%downlink consists of an expression that must evaluate to a net
%reference (usually a variable), a colon (:), the name of the
%channel, and an optional list of arguments. On the other side, the
%transition must be inscribed with an \emph{uplink}, which serve
%requests for everyone. Generally, transitions with an uplink cannot
%fire without being requested explicitly by another transition with a
%matching downlink. A transition has both uplink and downlinks, and
%may have multiple downlinks. Channels can also take a list of
%parameters. Although there is a direction of invocation, this
%direction need not coincide with the direction of information
%transfer. Indeed, it is possible that a single synchronisation
%transfers information in both directions.

In order to illustrate the main concepts of Reference nets,
Figure~\ref{introRenew} depicts a Reference net model that
represents a {\tt Resource Consumer} and two {\tt Resource
providers}, each of them with allocating capacity of two
resources. Services are required with a QoS and
data to be processed when {\tt Consumer} invokes the {\tt match}
channel. Communication happens when unification of variables is
possible. In the state represented in the figure, transition
labelled with the downlink {\tt this:match} channel in the {\tt Consumer}
 may synchronise with transitions labelled with uplinks {\tt :match}  in the {\tt Resource Provider 1}   and {\tt Resource Provider 2}  .

%\begin{figure}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \centering   \includegraphics[width=0.8\columnwidth]{images/consumerProviders.eps} \caption{A Reference net model that represents a {\tt Service Consumer} and two {\tt Resource Providers}. References to  {\tt Resources} net instances are managed by consumers and providers.}
%\label{introRenew}
%\end{figure}
%
%The unification between the channel variables gives
%the following possible firing modes:
%
%\begin{itemize}
%\item Synchronized firing modes of {\tt Consumer} with {\tt Resource Provider 1}:
%\begin{itemize}
%\item   {\tt request=serv1, QoS=2, inputData=data1, resource=resource[14] } and   {\tt request=serv2, QoS=2,  inputData=data2, resource=resource[14]}
%\item  {\tt service=serv1} or {\tt service=serv2, QoS=2, res=resource[14]}
%\end{itemize}
%
%\item Synchronized firing modes of {\tt Consumer} with {\tt Resource Provider 2}:
%\begin{itemize}
%\item  {\tt request=serv2, QoS=2, inputData=data2, resource=resource[10]} \\ or  {\tt resource[12]}  and \\   {\tt request=serv3, QoS=2,  inputData=data3, resource=resource[10]} \\ or   {\tt resource[12]}
%\item   {\tt service=serv2, QoS=2, res=resource[10]} or  {\tt res=resource[12]} \\ and {\tt service=serv3, QoS=2, res=resource[10]} or {\tt  res=resource[12]}
%\end{itemize}
%
%\end{itemize}
%
%The firing of these synchronized transitions provides the {\tt Consumer} with a
%reference to the
%{\tt resource} instance that will execute the service. The {\tt Consumer}
%may execute the service and recover the result synchronizing with the {\tt :begin} and {\tt :end}
%channels of the resource, once the {\tt Resource Provider} has allocated the resource. The resource Provider allocates and liberates the resource synchronization with the  {\tt :allocate} and {\tt free} channels, respectively.

Renew~\footnote{{\tt http://www.renew.de}}~\cite{DBLP:conf/apn/KummerWDSKMRV04} is a Java-based Reference net interpreter and a Reference net graphical modeling tool used in this work.
Petri nets and Reference nets have been used for specifying
scientific workflows~\cite{adaptiveExcpHand09,tolosanachpnt09}.
Reference nets along with Java inscriptions have been
used for implementing a service-oriented workflow engine,
DVega~\cite{DBLP:conf/otm/Tolosana-CalasanzBAE07}.



==> files/OldConclusion.tex <==
%


Analysis of formal model and experiments.

Simulations of complex scenarios

Metrics about the life-cycle

Monitoring and controlling a Kubernetes Cluster

\color{red}
A performance model for Kubernetes based deployment is outlined. With emerging interest in applications (such as stream processing) which need to launch and terminate instances on a per second basis, the overhead associated with VMs remains a limitation. We use a benchmark-based approach to better characterise behaviour of a Kubernetes system (using Docker containers). We propose a Reference net-based model for Pod \& container lifecycle in Kubernetes. Such a model can be used as a basis to support: (i) capacity planning and resource management; (ii) application design, specifically how an application may be structured in terms of pods and containers. Our future work involves undertaking further analysis on the model to study its properties and infer potential behaviours to support application scaling. 
\color{black}

%\begin{figure}
%\centering
%		\includegraphics[width=1.0\textwidth]{board.pdf}
%
%\end{figure} 


